Xorbits: Automating Operator Tiling for Distributed Data Science

Data science pipelines commonly utilize dataframe and array operations for tasks such as data preprocessing, analysis, and machine learning. The most popular tools for these tasks are pandas and NumPy. However, these tools are limited to executing on a single node, making them unsuitable for processing large-scale data. Several systems have attempted to distribute data science applications to clusters while maintaining interfaces similar to single-node libraries, enabling data scientists to scale their workloads without significant effort. However, existing systems often struggle with processing large datasets due to Out-of-Memory (OOM) problems caused by poor data partitioning. To overcome these challenges, we develop Xorbits, a high-performance, scalable data science framework specifically designed to distribute data science workloads across clusters while retaining familiar APIs. The key differentiator of Xorbits is its ability to dynamically switch between graph construction and graph execution. Xorbits has been successfully deployed in production environments with up to 5k CPU cores. Its applications span various domains, including user behavior analysis and recommendation systems in the e-commerce sector, as well as credit assessment and risk management in the finance industry. Users can easily scale their data science workloads by simply changing the import line of their pandas and NumPy code. Our experiments demonstrate that Xorbits can effectively process very large datasets without encountering OOM or data-skewing problems. Over the fastest state-of-the-art solutions, Xorbits achieves an impressive 2.66* speedup on average. In terms of API coverage, Xorbits attains a compatibility rate of 96.7%, surpassing the fastest framework by an impressive margin of 60 percentage points. Xorbits is available at https://github.com/xorbitsai/xorbits.

==> tile.tex <==
\section{Operator Dynamic Tiling}
\label{sec:operator_dynamic_tiling}

In this section, we first describe the three types of computation graphs (Section~\ref{subsec:computation_graph}) and how to build graphs dynamically utilizing runtime metadata (Section~\ref{subsec:adaptive_graph}).

\subsection{Computation Graph}
\label{subsec:computation_graph}

There are three different types of computation graphs in Xorbits: the tileable graph, the chunk graph, and the subtask graph. The three types of graphs are depicted in Figure~\ref{fig:computation_graph}. It is a data science pipeline that first reads files with \texttt{read\_parquet} and then executes \texttt{groupby.agg}. Note that Figure~\ref{fig:computation_graph} is only for illustration purposes; the real graphs may have far more nodes than this one. Generally, every Xorbits API exposed to users is internally defined as an operator, which appears as a circle in the computation graphs. And squares are data placeholders. In this case, the \texttt{xorbits.pandas.read\_parquet} operation is implemented as the \texttt{ReadParquet} operator. Three fundamental methods: \texttt{\_\_call\_\_}, \texttt{tile}, and \texttt{execute} should be implemented for each operator. These three methods correspond to the tileable graph, the chunk graph, and the subtask graph, respectively.

\textbf{Tileable graph}. By calling the \texttt{\_\_call\_\_} method on the client, the API provided to users is transformed into a node of the tileable graph. The tileable graph is a collection of all the operations defined by users and is the logical plan. It is not partitioned into multiple chunks yet.

\textbf{Chunk graph}. The tileable graph is then submitted to the supervisor, where every operator's \texttt{tile} method will be invoked. The \texttt{tile} method divides the data into multiple chunks according to the data size or other cues. For complex operators like \texttt{groupby.agg}, the \texttt{tile} method also adds internal nodes (i.e., the GroupbyAgg::map, Concat, and GroupbyAgg:agg nodes in Figure~\ref{fig:computation_graph} corresponding to the map, combine, and reduce stages, respectively). The map stage ingests the upstream chunk data and produces intermediate key-value pairs. The combine stage is a pre-aggregation phase that combines a subset of chunks. Unlike the MapReduce programming model that uses persistent storage to store the key-value pairs, Xorbits is an in-memory computing engine, and all the intermediate results are in our shared memory storage service. We add the combine stage to avoid too many chunks aggregating into a single worker node, which may lead to memory overflow. In some cases where we need to aggregate a lot of nodes, pre-aggregating can also improve performance. The reduce stage will aggregate and convert the key-value pairs into the actual result. Note that each operator has its own semantics, and not all operators would use the aforementioned map-combine-reduce stages.

\textbf{Subtask graph}. The subtask graph is the physical execution plan. It is optimized from the chunk graph. The subtask graph and the chunk graph are nearly identical, with the following exceptions: 1) nearby nodes in the chunk graph are fused to a subgraph called subtask; 2) every subtask in the graph is assigned with scheduling information indicating which worker it should run on. In Figure~\ref{fig:computation_graph} the \texttt{ReadParquet} and the \texttt{GroupbyAgg::map} are fused to form a subgraph, which will be scheduled to a particular worker. We will discuss the details of the fusion optimization in Section~\ref{sec:optimization}. The \texttt{execute} method is called on the workers, where the single-node Python package is executed to calculate the result given the split chunk. NumPy and CuPy are for the array API; pandas and cuDF are for the dataframe API; or any other Python libraries that need to scale to multiple nodes like HuggingFace's datasets, XGBoost, LightGBM, or statsmodels, etc. Note that each kind of circle node in the graph has a corresponding execution implementation.



\subsection{Accuracy}
\label{subsec:accuracy}

